Constructive Safety Control

This paper proposes a constructive approach to safety control of nonlinear cascade systems subject to multiple state constraints. New design ingredients include a unified characterization of safety and stability for systematic designs of safety controllers, and a novel technique of reshaping the feasible sets of quadratically constrained quadratic programming induced from safety control. The proposed method guarantees Lipschitz continuity of virtual control laws, enabling a stepwise constructive design. A refined nonlinear small-gain synthesis is employed to address the nonlinear uncertain interconnections between the resulting subsystems corresponding to different virtual control laws, and to guarantee the achievement of the safety control objective. When the safety constraints are removed, the proposed approach coincides with the standard constructive nonlinear control. The proposed safety-control algorithm is experimentally validated in a testbed involving a vertical takeoff and landing (VTOL) vehicle taking off in narrow spaces.

==> fig/fig_block_diagram_VTOL.tex <==
\begin{tikzpicture}
% Safety Controller and Reference-Tracking Controller Regions
\draw[rounded corners=4pt, dashed, fill=cyan!5]  (-7.9,1.7) rectangle (-1.3,-1);
\draw[rounded corners=4pt, dashed, fill=gray!5]  (-0.8,1.7) rectangle (5,-1);

% Linearized VTOL Dynamics Region
\draw[rounded corners=4pt, fill=gray!10, line width=0.75pt] (3.4,0.6) rectangle (4.8,-0.8);
\node at (4.1,0.1) {VTOL};
\node at (4.1,-0.3) {\eqref{eq_plant}};

% Safety Controller Region
\draw[rounded corners=4pt, fill=cyan!30, line width=0.75pt] (-7.7,0.5) rectangle (-1.5,-0.7);

% Reference-Tracking Controller Region
\draw[rounded corners=4pt, fill=green!10, line width=0.75pt] (-0.6,0.7) rectangle (2.4,-0.8);

% Dynamic state feedback law
\node[align=center] at (0.9,0) {Dynamic state\\ feedback law \eqref{eq_dynamic_feedback}};
\draw[-latex] (3.4,-0.3) -- (2.4,-0.3);

% Arrows and labels
\draw[-latex] (2.4,0.2) -- (3.4,0.2);
\node at (2.9,0.4) {$a_1,a_2$};
\node at (2.9,-0.6) {$\theta, \dot{\theta}$};
\node at (4.1,-1.4) {$x_1,x_2,x_3,x_4$};

% Operator Symbols
\node[align=left] at (-5,1.1) {Safety  Controller \eqref{eq_safety_control_law_varrhoL} \\ Reference-Tracking Controller \eqref{eq_reference_tracking_controller}};
\node at (1.2,1.2) {Linearized VTOL \eqref{eq_VTOL_dynamics2}};
\node at (-4.6,-0.1) {$u=\varrho_4(x_4-\varrho_3(x_3-\varrho_2(x_2-\varrho_1(x_1))))$};
\draw[-latex] (-1.3,0.3) -- (-0.8,0.3);
\draw[-latex] (5,0.3) -- (5.3,0.3) -- (5.3,-1.8) -- (-8.2,-1.8) -- (-8.2,0.3)-- (-7.9,0.3);
\node at (-1.1,0.7) {$u$};
\end{tikzpicture}


==> fig/fig_block_diagram_high_relative.tex <==
\begin{tikzpicture}
\draw[rounded corners=4pt, dashed, fill=cyan!5]  (-10.1,1.7) rectangle (-7.5,-0.9);
\draw[rounded corners=4pt, dashed, fill=cyan!5]  (-6.9,1.7) rectangle (-0.5,-0.9);

% Rectangle for Plant
\draw[rounded corners=4pt, fill=gray!10, line width=0.75pt] (0,0.7) rectangle (1.4,-0.7);
% Node and equation label for Plant
\node at (0.7,0.2) {Plant};
\node at (0.7,-0.2) {\eqref{eq_plant}};

% Rectangle for Safety Control Law 1
\draw[rounded corners=4pt, fill=cyan!30, line width=0.75pt] (-9.4,0.7) rectangle (-8,-0.7);
% \node at (-8.7,-0.2) {\eqref{eq_safety_control_law_varrhoL}};

% Rectangle for Safety Control Law 2
\draw[rounded corners=4pt, fill=cyan!30, line width=0.75pt] (-6,0.7) rectangle (-4.6,-0.7);
% \node at (-5.3,-0.2) {\eqref{eq_safety_control_law_varrhoL}};

% Rectangle for Safety Control Law 3
\draw[rounded corners=4pt, fill=cyan!30, line width=0.75pt] (-2.3,0.7) rectangle (-0.9,-0.7);
% \node at (-1.6,-0.2) {\eqref{eq_safety_control_law_varrhoL}};

% Arrows and labels
\draw[-latex] (-0.9,0) -- (0,0);
\node at (-0.3,0.3) {$u$};

\draw[-latex] (1.4,0.5) -- (2.1,0.5) -- (2.1,-2.1) -- (-9.7,-2.1) -- (-9.7,0) -- (-9.4,0);
\node at (-9.9,-1.8) {$x_1$};

% Ellipse for x_2
\draw (-6.4,0) ellipse (0.1 and 0.1);
\draw[-latex] (-8,0) -- (-6.5,0);

% Arrows for x_2, x_3, ..., x_n
\draw[-latex] (1.4,0.3) -- (1.9,0.3) -- (1.9,-1.8) -- (-6.4,-1.8) -- (-6.4,-0.1);
\draw[-latex] (-6.3,0) -- (-6,0);
\draw[-latex] (-4.6,0) -- (-4.1,0);
\draw[-latex] (-2.9,0) -- (-2.3,0);
\draw (-3,0) ellipse (0.1 and 0.1);
\draw[-latex] (1.4,-0.4) -- (1.7,-0.4) -- (1.7,-1.5) -- (-3,-1.5) -- (-3,-0.1);
\draw[-latex] (-3.6,0) -- (-3.1,0);

% Additional labels and ellipses
\node at (-3.8,0) {$\cdots$};
\node at (-6.7,-1.6) {$x_2$};
\node at (-3.4,-1.3) {$x_n$};
\node at (-8.7,0) {$\varrho_1(x_1)$};
\node at (-5.3,0) {$\varrho_2(\tilde{x}_2)$};
\node at (-1.6,0) {$\varrho_n(\tilde{x}_n)$};

% Nodes for x^* and \tilde{x}
\node at (-7.2,0.3) {$x^*_2$};
\node at (-6.3,0.3) {$\tilde{x}_2$};
\node at (-4.3,0.3) {$x^*_3$};
\node at (-3.4,0.3) {$x^*_n$};
\node at (-2.6,0.3) {$\tilde{x}_n$};

% Operator Symbols
\node at (-6.5,-0.4) {$+$};
\node at (-3.1,-0.4) {$+$};
\node at (-6.7,-0.2) {$-$};
\node at (-3.4,-0.2) {$-$};
\node at (1.6,0.1) {$\vdots$};
\node[align=left] at (-8.8,1.2) {Safety \\ Controller \eqref{eq_safety_control_law_varrhoL}};
\node[align=left] at (-4,1.2) {Reference-Tracking Controller \eqref{eq_reference_tracking_controller}};
\end{tikzpicture}


==> fig/fig_block_diagram_high_relative_dgree.tex <==
\begin{tikzpicture}
\draw[rounded corners=4pt, dashed, fill=cyan!5]  (-10.1,1.7) rectangle (-7.5,-0.9);
\draw[rounded corners=4pt, dashed, fill=cyan!5]  (-6.9,1.7) rectangle (-0.5,-0.9);

% Rectangle for Plant
\draw[rounded corners=4pt, fill=gray!10, line width=0.75pt] (0,0.7) rectangle (1.4,-0.7);
% Node and equation label for Plant
\node at (0.7,0.2) {Plant};
\node at (0.7,-0.2) {\eqref{eq_plant}};

% Rectangle for Safety Control Law 1
\draw[rounded corners=4pt, fill=cyan!30, line width=0.75pt] (-9.4,0.7) rectangle (-8,-0.7);
% \node at (-8.7,-0.2) {\eqref{eq_safety_control_law_varrhoL}};

% Rectangle for Safety Control Law 2
\draw[rounded corners=4pt, fill=cyan!30, line width=0.75pt] (-6,0.7) rectangle (-4.6,-0.7);
% \node at (-5.3,-0.2) {\eqref{eq_safety_control_law_varrhoL}};

% Rectangle for Safety Control Law 3
\draw[rounded corners=4pt, fill=cyan!30, line width=0.75pt] (-2.3,0.7) rectangle (-0.9,-0.7);
% \node at (-1.6,-0.2) {\eqref{eq_safety_control_law_varrhoL}};

% Arrows and labels
\draw[-latex] (-0.9,0) -- (0,0);
\node at (-0.3,0.3) {$u$};

\draw[-latex] (1.4,0.5) -- (2.1,0.5) -- (2.1,-2.1) -- (-9.7,-2.1) -- (-9.7,0) -- (-9.4,0);
\node at (-9.9,-1.8) {$x_1$};

% Ellipse for x_2
\draw (-6.4,0) ellipse (0.1 and 0.1);
\draw[-latex] (-8,0) -- (-6.5,0);

% Arrows for x_2, x_3, ..., x_n
\draw[-latex] (1.4,0.3) -- (1.9,0.3) -- (1.9,-1.8) -- (-6.4,-1.8) -- (-6.4,-0.1);
\draw[-latex] (-6.3,0) -- (-6,0);
\draw[-latex] (-4.6,0) -- (-4.1,0);
\draw[-latex] (-2.9,0) -- (-2.3,0);
\draw (-3,0) ellipse (0.1 and 0.1);
\draw[-latex] (1.4,-0.4) -- (1.7,-0.4) -- (1.7,-1.5) -- (-3,-1.5) -- (-3,-0.1);
\draw[-latex] (-3.6,0) -- (-3.1,0);

% Additional labels and ellipses
\node at (-3.8,0) {$\cdots$};
\node at (-6.7,-1.6) {$x_2$};
\node at (-3.4,-1.3) {$x_n$};
\node at (-8.7,0) {$\varrho_1(x_1)$};
\node at (-5.3,0) {$\varrho_2(\tilde{x}_2)$};
\node at (-1.6,0) {$\varrho_n(\tilde{x}_n)$};

% Nodes for x^* and \tilde{x}
\node at (-7.2,0.3) {$x^*_2$};
\node at (-6.3,0.3) {$\tilde{x}_2$};
\node at (-4.3,0.3) {$x^*_3$};
\node at (-3.4,0.3) {$x^*_n$};
\node at (-2.6,0.3) {$\tilde{x}_n$};

% Operator Symbols
\node at (-6.5,-0.4) {$+$};
\node at (-3.1,-0.4) {$+$};
\node at (-6.7,-0.2) {$-$};
\node at (-3.4,-0.2) {$-$};
\node at (1.6,0.1) {$\vdots$};
\node[align=left] at (-8.8,1.2) {Safety \\ Controller \eqref{eq_safety_control_law_varrhoL}};
\node[align=left] at (-4,1.2) {Reference-Tracking Controller \eqref{eq_reference_tracking_controller}};
\end{tikzpicture}


==> fig/fig_block_diagram_relative_one.tex <==
\begin{tikzpicture}
% Placeholder node at (0.1,0)
\node at (0.2,0) {};

% Rectangle for Plant
\draw[rounded corners=4pt, fill=gray!10, line width =0.75pt]  (0.7,0.7) rectangle (2.3,-0.7);
% Node and equation label for Plant
\node[align=center] at (1.5,0) {Plant\\ \eqref{eq_model_relative_degree_one}};

% Rectangle for Safety Control Law
\draw[rounded corners=4pt, fill=cyan!30, line width =0.75pt]  (-3.8,0.7) rectangle (-0.4,-0.7);
% Node and equation label for Safety Control Law
\node[align=center] at (-2.1,0) {Safety Controller \\ \eqref{eq_safety_control_law}};

% Rectangle for Nominal Controller
\draw[rounded corners=4pt, fill=cyan!30, line width =0.75pt]  (-8.1,0.7) rectangle (-4.7,-0.7);
\node[align=center] at (-6.4,0) {Nominal Controller\\ $\varrho_r(x)$};

% Arrows and labels
\draw[-latex] (-0.4,0) -- (0.7,0);
\node at (-0.1,0.2) {$u$};

\node at (-0.1,-0.3) {$w$};
\node at (-5.1,1.1) {$z$};

\draw[-latex] (2.3,0) -- (3,0) -- (3,-1.2) -- (-6.4,-1.2) -- (-6.4,-0.7);
\draw[-latex] (0.2,-0.3) -- (0.7,-0.3);
\node at (2.6,0.2) {$x$};


\draw (-2.1,-1.2) -- (-2.1,-0.7);
\draw [fill=black] (-2.1,-1.2) ellipse (0.05 and 0.05);
\draw [fill=black] (-4.2,1.1) ellipse (0.05 and 0.05);
\draw[-latex] (-4.7,-0.3) -- (-3.8,-0.3);

\draw[-latex]  (-4.2,1.1) -- (-4.2,0.3) -- (-3.8,0.3);
\draw[-latex]  (-4.8,1.1) -- (0.2,1.1) -- (0.2,0.4) -- (0.7,0.4);
\end{tikzpicture}

